ODE Test Problems: a MATLAB suite of initial value problems

ODE Test Problems (OTP) is an object-oriented MATLAB package offering a broad range of initial value problems which can be used to test numerical methods such as time integration methods and data assimilation (DA) methods. It includes problems that are linear and nonlinear, homogeneous and nonhomogeneous, autonomous and nonautonomous, scalar and high-dimensional, stiff and nonstiff, and chaotic and nonchaotic. Many are real-world problems from fields such as chemistry, astrophysics, meteorology, and electrical engineering. OTP also supports partitioned ODEs for testing IMEX methods, multirate methods, and other multimethods. Functions for plotting solutions and creating movies are available for all problems, and exact solutions are provided when available. OTP is desgined for ease of use-meaning that working with and modifying problems is simple and intuitive.

==> logo.tex <==
\thispagestyle{empty}
\setcounter{page}{0}

\makeatletter
\def\Year#1{%
  \def\yy@##1##2##3##4;{##3##4}%
  \expandafter\yy@#1;%
}
\makeatother

\begin{Huge}
\begin{center}
Computational Science Laboratory Technical Report CSL-TR-\Year{2019}-1 \\
\today
\end{center}
\end{Huge}
\vfil
\begin{huge}
\begin{center}
Steven Roberts, Andrey A Popov, and Adrian Sandu
\end{center}
\end{huge}

\vfil
\begin{huge}
\begin{it}
\begin{center}
ODE Test Problems: a MATLAB suite of initial value problems.
\end{center}
\end{it}
\end{huge}
\vfil


\begin{large}
\begin{center}
Computational Science Laboratory \\
``Compute the Future!'' \\[12pt]
Computer Science Department \\
Virginia Polytechnic Institute and State University \\
Blacksburg, VA 24060 \\
Phone: 1--(540)--231--2193 \\
Fax: 1--(540)--231--6075 \\ 
Email: \url{sandu@cs.vt.edu} \\
Web: \url{http://csl.cs.vt.edu}
\end{center}
\end{large}

\vspace*{1cm}


% \begin{tabular}{cp{1in}c}
% \raisebox{0pt}{\includegraphics[width=1.65in]{CSL_Logo.jpg}}
% &&
% \raisebox{0pt}{\includegraphics[width=2.0in,angle=270]{VTlogo_2018.pdf}} 
     %   \end{tabular}


% \begin{figure}[h!]
%   \minipage{0.45\textwidth}%
%   \includegraphics[width=0.45\textwidth]{CSL_Logo.png}%
%   \endminipage\hfill%
%   \minipage{0.45\textwidth}%
%   \includegraphics[width=0.45\textwidth,angle=270]{VTlogo_2018.pdf}%
%   \endminipage\hfill%
% \end{figure}

\begin{center}
  \includegraphics[width=0.90\textwidth]{{CSLVTlogo2018.png}}%
\end{center}

\newpage

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "TR"
%%% End:


==> problems/bpe.tex <==
\subsection{Boussinesq Paradigm Equation (BPE)}

A more complex Partial differential equation problem

\begin{align}
  u_{tt} = \Delta\left[u + \beta_1 u_{tt} - \beta_2\Delta u + \alpha f(u)\right]
\end{align}
with $f$ being some arbitrary function, typically a polynomial.

Assuming a spatial discretization on the Laplacian, set $\*M = \*I-\beta_1\*\Delta$, and rewrite
\begin{align}
  \*v &= \*M \*u\\
  \*v_{tt} &= \*\Delta\left[\*u -\beta_2 \*\Delta \*u + \alpha \*f(\*u)\right]
\end{align}
which we can write as a first order ODE:
\begin{align}
  \*y &= \begin{bmatrix}\*u\\\*u_t\end{bmatrix}\\
  \*y_t &= \begin{bmatrix}\*u_t\\ \*M^{-1}\*v_{tt}\end{bmatrix}
\end{align}

\getpresettable{bpe}
